Towards Unbiased BFS Sampling

Breadth First Search (BFS) is a widely used approach for sampling large unknown Internet topologies. Its main advantage over random walks and other exploration techniques is that a BFS sample is a plausible graph on its own, and therefore we can study its topological characteristics. However, it has been empirically observed that incomplete BFS is biased toward high-degree nodes, which may strongly affect the measurements. In this paper, we first analytically quantify the degree bias of BFS sampling. In particular, we calculate the node degree distribution expected to be observed by BFS as a function of the fraction f of covered nodes, in a random graph RG(pk) with an arbitrary degree distribution pk. We also show that, for RG(pk), all commonly used graph traversal techniques (BFS, DFS, Forest Fire, Snowball Sampling, RDS) suffer from exactly the same bias. Next, based on our theoretical analysis, we propose a practical BFS-bias correction procedure. It takes as input a collected BFS sample together with its fraction f. Even though RG(pk) does not capture many graph properties common in real-life graphs (such as assortativity), our RG(pk)-based correction technique performs well on a broad range of Internet topologies and on two large BFS samples of Facebook and Orkut networks. Finally, we consider and evaluate a family of alternative correction procedures, and demonstrate that, although they are unbiased for an arbitrary topology, their large variance makes them far less effective than the RG(pk)-based technique.

==> Facebook_results.tex <==

\section{\label{sec:Facebook}Real life example: Sampling of Facebook}
In this section we apply and test the previous ideas in a real-life large-scale system - the Facebook social graph.
With 250+ millions of active users, Facebook is currently the largest online social network. Crawling the entire topology of Facebook would require downloading about $50TB$ of HTML data~\cite{Gjoka2010}, which makes sampling a very practical alternative.
%Therefore, in practice, people either study complete datasets of particular Facebook networks (communities), or sample Facebook, typically using BFS-like techniques as in \cite{Wilson09}.


\subsection{Data collection}
We have implemented a set of crawlers to collect the samples of Facebook (FB)
%% In the camera ready there should be an ACK to Minas for that.
according to the UNI, BFS, RW, MHRW techniques.
The details of our implementation are described in~\cite{Gjoka2010}.
The data sets are summarized in Table~\ref{tab:Facebook_Datasets}.
%, where $|S|$ and $f$ are the absolute and relative lengths of the collected samples, respectively.

{\em UNI} is a true uniform sample of FB users (see~\cite{Gjoka2010} for details).
%It was obtained by uniformly sampling the entire FB userID space and discarding non allocated userIDs. This is a trivial version of rejection sampling and guarantees a uniform sampling of the existing users, regardless of their actual distribution in the userID space.
%, \ie even if there are gaps or non continuous allocation of IDs.
%We do not have a ground truth values of real node degree distribution $p_k$ or average node degree $\langle k\rangle$. Instead, we use UNI as a reference point.
%Although not perfect,
Thanks to a large number of samples~$|S|$, UNI gives a high quality estimation of $p_k$ and $\langle k\rangle$. Therefore, we use UNI as ground truth for comparison of various techniques.
%Indeed, the variance of the UNI estimator (\ref{eq:Ek_UNI}) of $\langle k\rangle$ can be shown to be
%$\Var_{\langle \widehat{k}\rangle} = \frac{1}{|S|-1} \sum_{v\in S}(k_v\!\!-\!\!\langle\widehat{k}\rangle)^2 = ??$

We ran two types of BFS crawling. BFS${}_{28}$ consists of 28 small BFS-es initiated at 28 randomly chosen nodes from UNI, which allowed us to easily parallelize the process. Moreover, at the time of data collection, we (naively) thought that this would reduce the BFS bias. After gaining more insight (which, nota bene, motivated this paper), we collected a single large BFS${}_{1}$, initiated at a randomly chosen node from UNI.
%\footnote{Strictly speaking, RW and MHRW were also collected in 28 independent runs. For simplicity, we interpret such 28 runs as a single long execution. This does not affect the results, because, in contrast to BFS, random walk forgets the initial node orders of magnitude faster than the crawl length we use.}
%The implementation of {\em RW} and {\em MHRW} is straightforward.



\begin{table}[t!]
  \centering
  {\footnotesize
\begin{tabular}{l|ccccc}
   & UNI              &   RW          &  BFS${}_{28}$   &  BFS${}_{1}$      & MHRW   \\
\hline
$|S|$              &  982K        & 2.26M & 28$\times$81K = 2.26M & 1.19M & 2.26M \\
%Total number of \textit{unique} users    &  982K \note{?}          & 2.19M         &  2.20M     & 1.19M  & 957K         \\
$f$  &  0.44\%           & 1.03\%         &  28$\times$0.04\%     & 0.54\%  & 1.03\%
%Crawling period                          &  04/22-04/30         & 05/03-05/08   & 04/30-05/03 &  \textcolor{blue}{??}&  04/18-04/23  \\
\end{tabular}}
  \caption{Facebook measurements - data set overview.}
  \label{tab:Facebook_Datasets}\vspace{-0.8cm}
\end{table}




\subsection{Results}
We present the Facebook sampling results in Table~\ref{tab:Facebook_degrees} and in Fig.~\ref{fig:Facebook_degree_disrtibutions}. The first row of Table~\ref{tab:Facebook_degrees} shows the average node degree $\langle k^*\rangle$ observed (sampled) by several techniques. The value sampled by UNI is $\langle k^*\rangle\eq 94.1$, which we interpret as the real value~$\langle k\rangle$. MHRW, as expected, recovers a similar value. In contrast RW and BFS are both biased towards high degrees by a factor larger than three!
The degree bias of RW is the largest. It drops very slightly under the (relatively very short) BFS${}_{28}$ crawl, which confirms our findings from~\ref{sec:Equivalence to RW}.
BFS${}_{1}$, a sample 15 times longer than BFS${}_{28}$, is significantly less biased, which is in agreement with~\ref{subsec:k^* is decreasing in f}.

The second row shows the \emph{expected} sampled average node degrees (\ie our predictions of the values in the first row), assuming that the underlying Facebook topology is a random graph $RG(p_k)$ with degree distribution $p_k$ equal to that sampled by UNI. As expected, this works very well for RW. However, the values predicted for BFS overshoot the reality. This is because Facebook \emph{is not} a pure random graph~$RG(p_k)$. For example, Facebook, as most social networks, is characterized by a high clustering coefficient~$c$.
We believe that it is possible to incorporate this fact in our analytical model, \eg by appropriately stretching the function $f(t)$ in Eq.~(\ref{eq:f(t)}). This is a main goal in our future work.

Finally, in the last row of Table~\ref{tab:Facebook_degrees} we apply the estimators developed in Section~\ref{sec:Correcting for node degree bias} to correct the degree biases of RW and BFS. 
%Avg degree: sampled (row 1), expected (row 2) and corrected (row 3) for various techniques. For each expected and corrected value, we give in parenthesis the formula used to compute it.
In the case of RW, the correction works very well.
%As expected, the BFS correction with the RW estimator (\ref{eq:Ek_est_RW}) underestimates $\langle k\rangle$ due to the non-replacement requirement.
For the BFS estimator, the results are significantly worse, clearly for the reasons discussed in the previous paragraph.

All the above observations hold also for the \emph{entire} degree distribution, which is shown in Fig.~\ref{fig:Facebook_degree_disrtibutions}.

\begin{table}
  \centering
  {\footnotesize
\begin{tabular}{l|ccccc}
   & UNI & RW & BFS${}_{28}$ & BFS${}_{1}$ & MHRW \\
  \hline
  $\langle k^*\rangle$ sampled & 94.1 & 338.0 & 323.9 & 285.9 & 95.2 \\
  $\langle k^*\rangle$ expected & - & 329.8 (\ref{eq:Ek_RW}) & 329.1 (\ref{eq:q_k_f}) & 328.7 (\ref{eq:q_k_f}) & 94.1 (\ref{eq:Ek_UNI}) \\
%  $\langle k^2\rangle\ /\ \langle k \rangle$ & 329.8 & - & - & - & - \\
%  $\langle\est{k}\rangle$ (\ref{eq:Ek_est_RW}) & - & 93.9 &  84.3 & 72.1 & - \\
  $\langle\est{k}\rangle$ estimated & - & 93.9 (\ref{eq:Ek_est_RW}) &  85.4 (\ref{eq:est{p}_k_BFS}) & 72.7 (\ref{eq:est{p}_k_BFS}) & 95.2 (\ref{eq:est_k_UNI})
%  $\langle\est{k}\rangle$  & - & - &   & - \\
\end{tabular}
}
\caption{ Facebook measurements - average node degree. In parenthesis we give the relevant equations.
% {\em E.g.}, ``329.1(11)'' means ``Eq.(11) computes a value of 11''.
}
\label{tab:Facebook_degrees}
%\vspace{-0.9cm}
\end{table}



\begin{figure}[t]
\psfrag{degree k}[c][b][0.9]{$k$\ \ node degree}
\psfrag{prob}[c][t][0.9]{Prob($k$)}
\psfrag{degreeDistr}[c][t][1]{Degree distributions sampled in Facebook}
\center
\includegraphics[width=0.4\textwidth]{figs/Facebook_degree_disrtibutions.eps}
\caption{{\bf Facebook measurements - degree distribution.} Crawlers used: UNI, RW and BFS. All plots are in log-log scale with logarithmic binning of data (we take the average of all points that fall in the same bin). We also correct these distributions, as described in Section~\ref{sec:Correcting for node degree bias}.}
\label{fig:Facebook_degree_disrtibutions}
%\vspace{-0.6cm}
\end{figure}


\subsection{Practical recommendations}
%Based on our analysis as well as on our experience with measuring Facebook, we summarize below some practical guidelines for using exploration techniques in practice.

BFS is strongly biased toward high degree nodes. It is possible to correct for this bias precisely when the underlying graph is a $RG(p_k)$ (which is not the case in practice). Also, in more realistic graphs, this bias can be corrected reasonably well for a very small sample size (as is the case for BFS${}_{28}$), where BFS is similar to RW (see Fig.~\ref{fig:contributions}).
On the other extreme, for very large sampling coverage, the bias of BFS becomes relatively small and could be sometimes neglected (even without additional correction).
However, in all other cases, the results become difficult to interpret.
In contrast, both RW (equipped with a correction procedure) and MHRW are unbiased, regardless of the actual graph topology. Therefore, we recommend using RW and MHRW (with a slight advantage of RW~\cite{Rasti09-RDS}) as general methods to sample the node properties.

In contrast, RW and MHRW are not useful when sampling \emph{non-local graph properties}, such as the graph diameter or the average shortest path length. In this case, BFS seems very attractive, because it produces a full view of a particular region in the graph, which is usually a densely connected graph itself, and for which the non-local properties can be easily calculated. However, all such results should be interpreted very carefully, as they may be also strongly affected by the bias of BFS. For example, the graph diameter (usually) drops significantly with growing average node degree of a network.

